Iwasawa theory of twists of elliptic modular forms over imaginary quadratic fields at inert primes

Our primary goal in this article is to study the Iwasawa theory for semi-ordinary families of automorphic forms on $\mathrm{GL}_2\times\mathrm{Res}_{K/\mathbb{Q}}\mathrm{GL}_1$, where $K$ is an imaginary quadratic field where the prime $p$ is inert. We prove divisibility results towards Iwasawa main conjectures in this context, utilizing the optimized signed factorization procedure for Perrin-Riou functionals and Beilinson--Flach elements for a family of Rankin--Selberg products of $p$-ordinary forms with a fixed $p$-non-ordinary modular form. The optimality enables an effective control on the $\mu$-invariants of Selmer groups and $p$-adic $L$-functions as the modular forms vary in families, which is crucial for our patching argument to establish one divisibility in an Iwasawa main conjecture in three variables.

==> preface.tex <==
%-----------------------------------------------------------------------------
% Beginning of preface.tex
%-----------------------------------------------------------------------------
%
% AMS-LaTeX 1.2 sample file for a monograph, based on amsbook.cls.
% This is a data file input by chapter.tex.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\chapter*{Preface}

This document is a sample prepared to illustrate the use of the
American Mathematical Society's \LaTeX{} document class
\texttt{amsbook} and publication-specific variants of that class.

This is an example of an unnumbered chapter which can be used for a Preface
or Foreword.

The purpose of this paper is to establish a relationship between an
infinite-dimensional Grassmannian and arbitrary algebraic vector bundles
of any rank defined over an arbitrary complete irreducible algebraic
curve, which generalizes the known connection between the Grassmannian
and line bundles on algebraic curves.

\aufm{Author Name}

%-----------------------------------------------------------------------------
% End of preface.tex
%-----------------------------------------------------------------------------

